Beyond Orthography: Automatic Recovery of Short Vowels and Dialectal Sounds in Arabic

This paper presents a novel Dialectal Sound and Vowelization Recovery framework, designed to recognize borrowed and dialectal sounds within phonologically diverse and dialect-rich languages, that extends beyond its standard orthographic sound sets. The proposed framework utilized a quantized sequence of input with(out) continuous pretrained self-supervised representation. We show the efficacy of the pipeline using limited data for Arabic, a dialect-rich language containing more than 22 major dialects. Phonetically correct transcribed speech resources for dialectal Arabic are scarce. Therefore, we introduce ArabVoice15, a first-of-its-kind, curated test set featuring 5 hours of dialectal speech across 15 Arab countries, with phonetically accurate transcriptions, including borrowed and dialect-specific sounds. We described in detail the annotation guideline along with the analysis of the dialectal confusion pairs. Our extensive evaluation includes both subjective -- human perception tests and objective measures. Our empirical results, reported with three test sets, show that with only one and half hours of training data, our model improve character error rate by ~ 7\% in ArabVoice15 compared to the baseline.

==> intro.tex <==
Self-supervised learning (SSL) paradigm has transformed speech research and technology, achieving remarkable performance \cite{} while reducing the dependency on extensively annotated datasets \cite{}. The SSL models
% information captured within these models demonstrates the capability to
excel at discerning the underlying acoustic properties in both frames \cite{} and utterance level \cite{} irrespective of language. Phonetic information are sailent and preserved even when these continuous representation are mapped to a finate set of codes via vector quantization \cite{Hsu2021, Sicherman2023,Wells2022,ElKheir2024}. These allows the learning paradigm to leverage unlabelled data to discover units capturing meaningful phonetic contrasts. The recent studies have exploited these quantized discrete units for either \textit{(i)} pretraining the SSL model \cite{baevski2020wav2vec, Hsu2021},  \textit{(ii)} acoustic unit discovery as a training objective \cite{VanNiekerk2020} or \textit{(iii)} even opt for such discrete labels for training ASR \cite{chang2023exploration} among others. 

% embaddings go through crude quantization \cite{}, in fact success of HuBERT \cite{} shows its effectiveness 
In this paper, we utilize the SSL representation and vector quantization to identify/recover acoustic units for phonologically rich spoken dialects that go beyond its standardized sound set backed in its orthography. We proposed a simple, yet effective network design utilizing SSL representation and a discrete codebook for recognizing these unwritten dialectal and borrowed sounds with limited labeled data. % , and generate true representative of the sound sequences. 
% Moreover, we introduce a test set of $5 hours$ of speech containing transcriptions of 15 Arabic dialects, including borrowed sounds and dialectal variations. 


% Yet, it is still to be seen, whether such representation can effectively identify/recover acoustic units for phonologically rich spoken dialects that go beyond its standardized sound set backed in its orthography. We proposed a simple, yet effective network design utilizing SSL representation and a discretized codebook to recognize these sounds and generate true representative sound sequences. Moreover, we introduce a test set of $5 hours$ of speech containing transcriptions of 15 Arabic dialects, including borrowed sounds and dialectal variations. 

Arabic is an appropriate language for the task. The language has a rich tapestry of dialects, each with its unique characteristics in phonology, morphology, syntax, and lexicon \cite{ali2021connecting}. These dialects\footnote{There are 22 Arab countries, and typically, there is more than one dialect spoken in each Arab country (ex: rural versus urban areas)} differ not only among themselves but also when compared to Modern Standard Arabic (MSA). While MSA prevails in official and educational domains, Dialectal Arabic (DA) serves as the means for daily communication. 
The diversity in pronunciation and phoneme sets for DA goes beyond standardized MSA sound sets. Moreover, to add to the challenges, dialectal Arabic follows no standard orthography. Therefore, despite the abundance of DA speech data in online platforms, accurately (phonetically correct) transcribed resource are scarce, categorizing DA as a low-resource language. % in terms of available annotated data.

% and phonetically correct written
% the written (and phonetically correct) transcript are often rare putting DA as low-resource category.


% these dialects have no 

Our research explores the fascinating phonological aspects of Arabic dialects, providing a detailed examination of their subtleties sounds and their influence on reading MSA. With the large number of Arabic dialects, the diversity in pronunciation and phoneme sets goes beyond standardized MSA sounds set. This study addresses the crucial challenge of identifying and understanding these phonetic intricacies, acknowledging their essential role in improving the performance of speech processing applications like dialectal Text-to-Speech (TTS) and Computer-Assisted Pronunciation Training applications. 


simple vector quantization of SSL e


study the SSL embeddings and its discritozation to understand the latent representation of dialectal units,



non-standard orthographic languages/dialects.\footnote{} 
However, it remains to determine if these representations are capable of identifying acoustic units with little to no manual annotation.

differentiating salient frame-level information discreminating different dialectal 
In this study, we aim to utilize these frame-level SSL representations to learn and recover different acoustic units for spoken dialectal Arabic. 

The fine-grained representations in SSL models are shown to capture the underlying acoustic units, discriminating them based on different properties 


Spoken DA remains a low-resource language primarily due to the scarcity of transcription that can faithfully capture the diverse regional and borrowed sounds in the standard written format. Automatically recognising the vowels, borrowed and dialectal sound 

==> msa_sounds.tex <==

Arabic dialects vary on many dimensions –
primarily, geography and social class. Geolinguistically, the Arab world can be divided in
many different ways. The following is only one
of many that covers the main Arabic dialects:
• Gulf Arabic (GLF) includes the dialects of
Kuwait, Saudi Arabia, Bahrain, Qatar, United
Arab Emirates, and Oman.
• Iraqi Arabic (IRQ) is the dialect of Iraq. In
some dialect classifications, Iraqi Arabic is
considered a sub-dialect of Gulf Arabic.
• Levantine Arabic (LEV) includes the dialects of  Syria, Lebanon, Jordan, and Palestine.
• Egyptian Arabic (EGY) covers the dialects
of the Nile valley: Egypt and Sudan.
• Maghrebi Arabic covers the dialects of
Algeria, Morocco, Tunisia, Libya, and Mauritania.
%Libya is sometimes included.
Yemenite Arabic is often considered its own
class. Maltese Arabic is not always considered an Arabic dialect. It is the only Arabic
variant that is considered a separate language
and is written with Latin script.

Although Arabic dialects and MSA vary on many
different levels — phonology, orthography, morphology, lexical choice and syntax — we will
focus on phonological difference in this paper.1
MSA’s phonological profile includes 28 consonants, three short vowels, three long vowels and
two diphthongs (/ay/ and /aw/). Arabic dialects
vary phonologically from standard Arabic and
each other. Some of the common variations include the following (Holes, 2004; Habash, 2006):
The MSA consonant (/q/) is realized as a glottal stop /’/ in EGY and LEV and as /g/ in GLF and
IRQ. For example, the MSA word \<طريق> /t
¯
ari:q/ ‘road’
appears as /t
¯
ari:’/ (EGY and LEV) and /t
¯
ari:g/ (GLF
and IRQ). Other variants also are found in sub dialects such as /k/ in rural Palestinian (LEV) and
/dj/ in some GLF dialects. These changes do not
apply to modern and religious borrowings from
MSA. For instance, the word for \<قرآن> ‘Qur’an’ is never
pronounced as anything but /qur’a:n/.
The MSA alveolar affricate (/dj/) is realized as
/g/ in EGY, as /j/ in LEV and as /y/ in GLF. IRQ
preserves the MSA pronunciation. For example,
the word \<جميل> for ‘handsome’ is /djami:l/ (MSA, IRQ),
/gami:l/ (EGY), /jami:l/ (LEV) and /yami:l/ (GLF).


The MSA consonant (/k/) is generally realized
as /k/ in Arabic dialects with the exception of GLF,
IRQ and the Palestinian rural sub-dialect of LEV,
which allows a /c/ pronunciation in certain con- ˇ
texts. For example, the word \<سمك> for ‘fish’ is /samak/
in MSA, EGY and most of LEV but /simac/ in IRQ
and GLF.
The MSA consonant /θ/ is pronounced as /t/ in
LEV and EGY (or /s/ in more recent borrowings
from MSA), e.g., the MSA word /θala:θa/ ‘three’
is pronounced /tala:ta/ in EGY and /tla:te/ in LEV.
IRQ and GLF generally preserve the MSA pronunciation.


The MSA consonant /δ/ is pronounced as /d/
in LEV and EGY (or /z/ in more recent borrowings from MSA), e.g., the word for ‘this’ is pronounced /ha:δa/ in MSA versus /ha:da/ (LEV) and
/da/ EGY. IRQ and GLF generally preserve the
MSA pronunciation.
The MSA consonants /d
¯
/ (emphatic/velarized
d) and /δ
¯
/ (emphatic /δ/) are both normalized to
/d
¯
/ in EGY and LEV and to /δ
¯
/ in GLF and IRQ.
For example, the MSA sentence /δ
¯
alla yad
¯
rubu/
‘he continued to hit’ is pronounced /d
¯
all yud
¯
rub/
(LEV) and /δ
¯
all yuδ
¯
rub/ (GLF). In modern borrowings from MSA, /δ
¯
/ is pronounced as /z
¯
/ (emphatic z) in EGY and LEV. For instance, the word
for ‘police officer’ is /δ
¯
a:bit
¯
/ in MSA but /z
¯
a:bit
¯
/
in EGY and LEV.
In some dialects, a loss of the emphatic feature
of some MSA consonants occurs, e.g., the MSA
word /lat
¯
i:f/ ‘pleasant’ is pronounced as /lati:f/ in
the Lebanese city sub-dialect of LEV. Emphasis typically spreads to neighboring vowels: if a
vowel is preceded or succeeded directly by an emphatic consonant (/d
¯
/, /s
¯
/, /t
¯
/, /δ
¯
/) then the vowel
becomes an emphatic vowel. As a result, the loss
of the emphatic feature does not affect the consonants only, but also their neighboring vowels.
Other vocalic differences between MSA and the
dialects include the following: First, short vowels change or are completely dropped, e.g., the
MSA word /yaktubu/ ‘he writes’ is pronounced
/yiktib/ (EGY and IRQ) or /yoktob/ (LEV). Second, final and unstressed long vowels are shortened, e.g., the word /mat
¯
a:ra:t/ ‘airports’ in MSA
becomes /mat
¯
ara:t/ in many dialects. Third, the
MSA diphthongs /aw/ and /ay/ have mostly become /o:/ and /e:/, respectively. These vocalic
changes, particularly vowel drop lead to different
syllabic structures. 

MSA syllables are primarily
light (CV, CV:, CVC) but can also be (CV:C and
CVCC) in utterance-final positions. EGY syllables are the same as MSA’s although without the
utterance-final restriction. LEV, IRQ and GLF allow heavier syllables including word initial clusters such as CCV:C and CCVCC. \textcolor{red}{examples?}


==> sounds_analysis.tex <==
\section{Sounds Analysis}
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{figures/labels2.png}
\caption{2D t-SNE Projection of Frame-Level Presentations Extracted Randomly from Finetuned Arabic XLS-R. A. Pairs (\<ز ذ>) \textipa[\dh \ z]. B. Sounds (\<ت ة ه>) \textipa[h t]. C. Pairs (\<چ ج>) \textipa[\textipa{d\textctz}\ g \textctz].}
\label{fig:dialects_samples}
\end{figure*}

In Figure \ref{fig:dialects_samples}, we illustrated various potential confusion between certain sounds in MSA and Arabic dialects. We employed a Hidden Markov Model-Time Delay Neural Network (HMM-TDNN) model\footnote{\url{https://kaldi-asr.org/models/m13}}, trained with MGB-2 \cite{ali2016mgb} for Arabic, to align randomly selected samples from the original datasets of CommonVoice Arabic and EgyAlj. In the case of the English dataset TIMIT, we utilized the provided ground truth alignment.

After aligning the speech signals with their corresponding original unvowelized character-based transcriptions, we matched the frame-level features extracted from XLS-R (see Section \ref{sec:xlsr}) with their characters. For Figure \ref{fig:dialects_samples}.A, we randomly chose $1000$ samples associated with \<ز> [\textipa{z}] and $1000$ samples associated with  \<ذ> [\textipa{\dh}] from CommonVoice Arabic. Even though CommonVoice Arabic is considered as MSA where pronunciation is considered to be good, we note that some samples \<ذ> [\textipa{\dh}] get into the cluster of \<ز> [\textipa{z}] mostly due to dialectal influence, as discussed in the previous literature in Section \ref{sec:arabsounds}. 

Figure \ref{fig:dialects_samples}.B represents the selection of three characters used: \<ت> [\textipa{t}], 
\<ة> [\textipa{t}/\textipa{h}], 
\<ه> [\textipa{h}]. When it comes to \<ة>, it is sometimes pronounced as [\textipa{t}] and sometimes as [\textipa{h}]. With some rule-based rules \cite{halabi2016phonetic}, we can recover when it will match which sound, yet for spoken quotidian, it is hard to apply these rules where people don't follow. The figure shows mainly two clusters for [\textipa{t}] and [\textipa{h}], and vectors associated with \<ة> get scattered between these two clusters, illustrating the previous point.

Figure \ref{fig:dialects_samples}.C represents the selection of four labels are used: Arabic \<ج> [ [\textipa{d\textctz}], 
and English phonemes [\textctz, \textipa{g}, \textipa{d\textctz}]. We selected Arabic samples \<ج> for CommonVoice Arabic and EgyAlj




% When it comes to \<ة>, it is sometimes pronounced as [\textipa{t}] and sometimes as [\textipa{h}]. With some rule-based rules \cite{halabi2016phonetic}, we can recover when it will match which sound, yet for spoken quotidian, it is hard to apply these rules where people don't follow. The figure shows mainly two clusters for [\textipa{t}] and [\textipa{h}], and vectors associated with \<ة> get scattered between these two clusters, illustrating the previous point.






% In Figure \ref{fig:dialects_samples}, we illustrated various dialectic variations and some potential confusion between certain sounds in MSA and Arabic dialects. We employed a Hidden Markov Model-Time Delay Neural Network (HMM-TDNN) model\footnote{\url{https://kaldi-asr.org/models/m13}}, trained with MGB-2 \cite{ali2016mgb} for Arabic, to align randomly selected samples from the original datasets of CommonVoice Arabic, and EgyAlj. In the case of the english dataset TIMIT, we utilized the provided ground truth alignment.

% After aligning the speech signals with their corresponding original unvowelized character-based transcriptions, we matched the frame-level features extracted from XLS-R \ref{sec:xlsr} with their characters. For Figure \ref{fig:dialects_samples}.A, we randomly chose $1000$ samples associated with \<ز> [\textipa{z}] and $1000$ samples associated with  \<ذ> [\textipa{\dh}] from CommonVoice Arabic. Eventhough that CommonVoice Arabic is considered as MSA where pronunication are considered to be good, we note that some sounds \<ذ> [\textipa{\dh}] get into the cluster of \<ز> [\textipa{z}] which is in the stream of previous literature in Section \ref{sec:arabsounds}. Figure \ref{fig:dialects_samples}.B represents the selection three characters used: \<ت> [\textipa{t}], 
% \<ة> [\textipa{t}/\textipa{h}], 
% \<ه> [\textipa{h}]. When it comes to \<ة>, sometimes it pronounced as [\textipa{t}] and sometimes [\textipa{h}], with some based-ruled we can guess when it will match which sound, yet for spoken quotidien, it  hard to apply these rules where people don't follow. The Figure shows majoraly two clusters, and vectors associated to \<ة> get scatter between these two clusters showing the previous point.


Lastly, Figure \ref{fig:dialects_samples}.C illustrates the English sounds zh, g, jh, paired with the Arabic sound dj.

% In Figure \ref{fig:dialects_samples}, we showed some common dialect variations and some confusion between some sounds in MSA and Arabic Dialects. We extracted features of randomly selected original samples from CommonVoice Arabic data and EgyAlj and TIMIT datasets after force-alignment using a grapheme based Hidden Markov Model-Time Delay Neural Network (HMM- TDNN) model \footnote{https://kaldi-asr.org/models/m13} trained with MGB-2 \cite{ali2016mgb} for Arabic, and we used the given ground truth alignment in TIMIT. 

% In Figure \ref{fig:dialects_samples}, we showed some common dialect variations and some confusion between some sounds in MSA and Arabic Dialects. Given randomly selected samples from original --unannotated dataset from CommonVoice Arabic, EgyAlj and TIMIT datasets, we force-aligned samples speech signal with the its corresponding grapheme based transcription using a Hidden Markov Model-Time Delay Neural Network (HMM- TDNN) model\footnote{\url{https://kaldi-asr.org/models/m13}} trained with MGB-2 \cite{ali2016mgb} for Arabic, and we used the given ground truth alignment in TIMIT. After the alignment, we matched the frame-level features extracted from XLS-R \ref{sec:xlsr}, with their labeling. For Figure \ref{fig:dialects_samples}.A, we randomly selected $1000$ samples associated with $z$, and $1000$ from $dh$ from CommonVoice Arabic and EgyAlj. For Figure \ref{fig:dialects_samples}. B, represents the three used characters t,h,t. and C represents the english sounds zh, g, jh with arabic dj. 







we extracted  using the the finetuned XLS-R as presented in Section \ref{sec:xlsr}. In figure A, 




In Figure \ref{fig:dialects_samples}, we illustrated various potential confusion between certain sounds in MSA and Arabic dialects. We employed a Hidden Markov Model-Time Delay Neural Network (HMM-TDNN) model\footnote{\url{https://kaldi-asr.org/models/m13}}, trained with MGB-2 \cite{ali2016mgb} for Arabic, to align randomly selected samples from the original datasets of CommonVoice Arabic and EgyAlj. In the case of the English dataset TIMIT, we utilized the provided ground truth alignment.

After aligning the speech signals with their corresponding original unvowelized character-based transcriptions, we matched the frame-level features extracted from XLS-R (see Section \ref{sec:xlsr}) with their characters. For Figure \ref{fig:dialects_samples}.A, we randomly chose $1000$ samples associated with \<ز> [\textipa{z}] and $1000$ samples associated with  \<ذ> [\textipa{\dh}] from CommonVoice Arabic. Even though CommonVoice Arabic is considered as MSA where pronunciation is considered to be good, we note that some samples \<ذ> [\textipa{\dh}] get into the cluster of \<ز> [\textipa{z}] mostly due to dialectal influence, as discussed in the previous literature in Section \ref{sec:arabsounds}. 

Figure \ref{fig:dialects_samples}.B represents the selection of three characters used: \<ت> [\textipa{t}], 
\<ة> [\textipa{t}/\textipa{h}], 
\<ه> [\textipa{h}]. When it comes to \<ة>, it is sometimes pronounced as [\textipa{t}] and sometimes as [\textipa{h}]. With some rule-based rules \cite{halabi2016phonetic}, we can recover when it will match which sound, yet for spoken quotidian, it is hard to apply these rules where people don't follow. The figure shows mainly two clusters for [\textipa{t}] and [\textipa{h}], and vectors associated with \<ة> get scattered between these two clusters, illustrating the previous point.

Figure \ref{fig:dialects_samples}.C represents the selection of four labels are used: Arabic \<ج> [ [\textipa{d\textctz}], 
and English phonemes (zh, g, jh) [\textctz, \textipa{g}, \textipa{d\textctz}]. We $1000$ samples selected Arabic samples \<ج> from CommonVoice Arabic and EgyAlj along with $500$ samples for each of the english phonemes. We noticed the Arabic \<ج> sound is scattered across different english pronunication zh, g, and jh. Which shows the dialectal variation of the pronunication of \<ج>. 

==> table_cer.tex <==
\begin{table}[!ht]
\centering
\begin{minipage}[t]{0.5\linewidth}
\scalebox{0.6}{
\begin{tabular}{l|ccc}
\toprule
\multicolumn{1}{c}{CER} & $Z$   & $D_D$   & $D_J$ \\ \midrule\midrule
\rowcolor{yellow!20}
\multicolumn{4}{c}{1hr 30min}                                                                           \\ \hline\hline
CV-                     & 0.113                 & 0.108                    & \textbf{0.094}           \\
EgyAlj                  & 0.252                 & \textbf{0.206}           & 0.231                    \\
AraVoice15              & 0.536                 & \textbf{0.447}           & 0.464                    \\ \hline
% Average        & 0.300      & \textbf{0.254}          & 0.263       \\ \hline\hline
\rowcolor{gray!20}
\multicolumn{4}{c}{3hrs 30min}                                                                           \\\hline\hline
CV-                     & 0.103                 & 0.108                    & \textbf{0.096}           \\
EgyAlj                  & 0.270                 & \textbf{0.241}           & 0.253                    \\
AraVoice15              & 0.497                 & \textbf{0.470}           & 0.483                    \\\hline
% \rowcolor{gray!20}
% \multicolumn{4}{c}{5hrs 30min}                                                                           \\\hline\hline
% CV-                     & \textbf{0.095}        & 0.110                    & 0.099                    \\
% EgyAlj                  & 0.257                 & \textbf{0.245}           & 0.248                    \\
% AraVoice15              & 0.485                 & \textbf{0.477}           & 0.491                    \\\hline
% \rowcolor{gray!20}
% \multicolumn{4}{c}{$\sim$20 hrs }                                                                      \\\hline\hline
% CV-                     & \textbf{0.099}        & 0.108                    & 0.101                    \\
% EgyAlj                  & 0.264                 & 0.244                    & \textbf{0.227}           \\
% AraVoice15              & 0.492                 & 0.478                    & \textbf{0.457}          
\end{tabular}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth} % Begin the right minipage
\centering
\scalebox{0.6}{
\begin{tabular}{l|ccc}
\toprule
\multicolumn{1}{c}{CER} & $Z$   & $D_D$   & $D_J$ \\ \midrule\midrule
% \rowcolor{yellow!20}
% \multicolumn{4}{c}{1hr 30min}                                                                           \\ \hline\hline
% CV-                     & 0.113                 & 0.108                    & \textbf{0.094}           \\
% EgyAlj                  & 0.252                 & \textbf{0.206}           & 0.231                    \\
% AraVoice15              & 0.536                 & \textbf{0.447}           & 0.464                    \\ \hline
% % Average        & 0.300      & \textbf{0.254}          & 0.263       \\ \hline\hline
% \rowcolor{gray!20}
% \multicolumn{4}{c}{3hrs 30min}                                                                           \\\hline\hline
% CV-                     & 0.103                 & 0.108                    & \textbf{0.096}           \\
% EgyAlj                  & 0.270                 & \textbf{0.241}           & 0.253                    \\
% AraVoice15              & 0.497                 & \textbf{0.470}           & 0.483                    \\\hline
\rowcolor{gray!20}
\multicolumn{4}{c}{5hrs 30min}                                                                           \\\hline\hline
CV-                     & \textbf{0.095}        & 0.110                    & 0.099                    \\
EgyAlj                  & 0.257                 & \textbf{0.245}           & 0.248                    \\
AraVoice15              & 0.485                 & \textbf{0.477}           & 0.491                    \\\hline
\rowcolor{gray!20}
\multicolumn{4}{c}{$\sim$20 hrs }                                                                      \\\hline\hline
CV-                     & \textbf{0.099}        & 0.108                    & 0.101                    \\
EgyAlj                  & 0.264                 & 0.244                    & \textbf{0.227}           \\
AraVoice15              & 0.492                 & 0.478                    & \textbf{0.457}          
\end{tabular}}
\end{minipage}
\caption{Reported CER performance for borrowed and dialectal unit recognition task with Baseline ($Z$), DVR Discrete ($D_D$) and DVR Joint ($D_J$) models, for all three test sets and different training data sizes.  }
\label{tab:cer}
\end{table}


 We observed for borrowed and dialectal unit recognition, the discrete model outperforms the joint model significantly.

  We see an improvement in performance from 1hr30min to 3hr30min settings. However, beyond a certain data threshold, the improvements plateaued. 
